From dense to sparse design: Optimal rates under the supremum norm for estimating the mean function in functional data analysis

We derive optimal rates of convergence in the supremum norm for estimating the H\"older-smooth mean function of a stochastic process which is repeatedly and discretely observed with additional errors at fixed, multivariate, synchronous design points, the typical scenario for machine recorded functional data. Similarly to the optimal rates in $L_2$ obtained in \citet{cai2011optimal}, for sparse design a discretization term dominates, while in the dense case the parametric $\sqrt n$ rate can be achieved as if the $n$ processes were continuously observed without errors. The supremum norm is of practical interest since it corresponds to the visualization of the estimation error, and forms the basis for the construction uniform confidence bands. We show that in contrast to the analysis in $L_2$, there is an intermediate regime between the sparse and dense cases dominated by the contribution of the observation errors. Furthermore, under the supremum norm interpolation estimators which suffice in $L_2$ turn out to be sub-optimal in the dense setting, which helps to explain their poor empirical performance. In contrast to previous contributions involving the supremum norm, we discuss optimality even in the multivariate setting, and for dense design obtain the $\sqrt n$ rate of convergence without additional logarithmic factors. We also obtain a central limit theorem in the supremum norm, and provide simulations and real data applications to illustrate our results.

==> MeanFunctionEstimationRates/Proofs/proofsbandwidth.tex <==
\begin{proof}
In Theorem \ref{theorem:estimation:rates} the convergence rate of the bias $I_1^{\bs p, h}$ is increasing in $h$ whereas for the error term $I_2^{n, \bs p, h}$ induced by noise it decreases. Hence, we obtain the optimal rate in total by balancing these two rates. If $ h \eqsim \big(\log(n\bs{p^1})/(n\bs{p^1})\big)^{1/(2\alpha+d)}$, it follows that
\begin{align*}
	\bigg(\frac{\log(1/h)}{n\,\bs{p^1}\,h^d}\bigg)^{\frac12} &\eqsim \bigg(\frac{\log(n\,\bs{p^1})}{n\,\bs{p^1}}\bigg)^{\frac{\alpha}{2\alpha+d}} \eqsim h^\alpha \, .
\end{align*}  
However, we have to guarantee $h=\Oop{\pmin^{-1} }$ because of Assumption \ref{ass:weights}, which results in 
\begin{equation*}
	h \eqsim \max \Bigg(\bigg(\frac{\log(n\bs{p^1})}{n\bs{p^1}}\bigg)^{\frac1{2\alpha+d}},\frac1{\pmin}\Bigg) \, .
\end{equation*}
Now, $\pmin^{-1} \gtrsim \big( \log(n\,\bs{p^1})/(n\,\bs{p^1})\big)^{1/(2\alpha+d)}$ is equivalent to the opposite of the condition in \eqref{eq:optimal:bandwidth} and, in consequence,
\begin{align*}
	\sqrt{ \frac{\log(\pmin)}{n\, \bs{p^1}/\pmin^d} } \lesssim \sqrt{\frac{\log(n\,\bs{p^1})}{n\,\bs{p^1} }} \cdot \pmin^{d/2} \lesssim \pmin^{-\alpha}\,.
\end{align*}
The result in i) then follows by the case distinction in $\pmin \lesssim n^{1/(2\alpha)}$.\\
If conversely, $\bs{p^1} \lesssim \log(n\,\bs{p^1})/n \, \pmin^{2\alpha+d}$ then the balancing bandwidth $h\eqsim \big( \log(n\,\bs{p^1})/(n\,\bs{p^1})\big)^{1/(2\alpha+d)}$ can be chosen. \\

If in addition it holds $\bs{p^1} \lesssim n^{1/(2\alpha)}\log(n\,\bs{p^1})$ then we get 
\begin{align*}
    \bigg( \frac{\log(n\,\bs{p^1})}{n\,\bs{p^1}} \bigg)^{\frac{\alpha}{2\alpha+d}} & 
    %\gtrsim \frac{\log(n ( \bs{p^1} - 1) )^{\frac{\alpha}{2\alpha+d}}}{\sqrt n} 
    \gtrsim \frac1{\sqrt n}\,,
\end{align*}
and vice versa.

% \begin{enumerate}
% 	\item In this case it is $h^\star\eqsim p_1^{-1}$, which in view of Theorem \ref{theorem:estimation:rates} leads to 
% 	\begin{align*}
% 		 \sup_{\mu\in\hclass\, Z \in \Pclass} \E_\mu \Big[ \normib{ \mulestar - \mu} \Big]
% %		\leq & \sup_{\mu\in\hclass} \normib{\Ionestar}
% %		+ \E  \Big[\normib{\Itwostar}  \Big]+\E  \Big[ \normib{\Ithreestar}  \Big] \\
% 		=& \Oop{ \max\bigg(p_1^{-\alpha}, \bigg(\frac{\log(p_1)}n\bigg)^{\frac12}, n^{-\frac12}\bigg) }
% 	\end{align*}
% 	by .
% 	Since
% 	\begin{align*}
% 		p_1^{-\alpha} \gtrneqsim \bigg(\frac{\log(n)}{n}\bigg)^{\frac12} \gtrneqsim n^{-\frac12} \qquad \text{and} \qquad	p_1^{-\alpha} &\gtrneqsim \bigg(\frac{\log(n)}{n}\bigg)^{\frac12} \gtrsim \bigg(\frac{\log(p_1)}{n}\bigg)^{\frac12} \,,
% 	\end{align*}
% 	if $p_1 \lessneqsim \big(n/\log(n)\big)^{1/(2\alpha)}$, the assertion follows.
	
% 	\item It is $h^\star \eqsim \big(\log(np_1)/(np_1)\big)^{1/(2\alpha+d)}$, and the rates of the bias and the error term induced by noise are balanced. Thus,
% 	\begin{align} \label{eq:rate:balanced}
% 		\sup_{\mu\in\hclass\, Z \in \Pclass} \E_\mu \Big[ \normib{ \mulestar - \mu} \Big] =  \Oop{ \max\bigg( \bigg(\frac{\log (n\bs{p^1})}{n\bs{p^1}}\bigg)^{\frac{\alpha}{2\alpha + d}}, n^{-\frac12}  \bigg) }
% 	\end{align}  
% 	by Theorem \ref{theorem:estimation:rates}. If $\big(n/\log(n)\big)^{1/(2\alpha)}\lesssim p_1\lesssim n^{1/(2\alpha)}\log(n)^{1/d}$, then $\log(p_1)\eqsim\log(n)$ and, in particular,
% 	\[\bigg(\frac{\log(n\bs{p^1})}{n\bs{p^1}}\bigg)^{\frac{\alpha}{2\alpha+d}} \eqsim \bigg(\frac{\log(n)}{n\bs{p^1}}\bigg)^{\frac{\alpha}{2\alpha+d}} \gtrsim \bigg(\frac{\log(n)}{n^{\frac{2\alpha+d}{2\alpha}}\log(n)}\bigg)^{\frac\alpha{2\alpha+d}}\eqsim  n^{-\frac12} \,,\]
% 	which gives the assertation.
	
% 	\item Since $(\log(n\bs{p^1})/n\bs{p^1}))^{\alpha/(2\alpha+d)}$ is strictly monotonically decreasing in $p_1$ we obtain
% 	\[\bigg(\frac{\log(n\bs{p^1})}{n\bs{p^1}}\bigg)^{\frac{\alpha}{2\alpha+d}}  \lessneqsim
% 	\bigg(\frac{\log\big(n^{\frac{2\alpha+d}{2\alpha}}\log(n) \big)}{n^{\frac{2\alpha+d}{2\alpha}}\log(n)}\bigg)^{\frac\alpha{2\alpha+d}} \eqsim \bigg(\frac{\log(n)}{n^{\frac{2\alpha+d}{2\alpha}} \log(n)}\bigg)^{\frac\alpha{2\alpha+d}} \eqsim n^{-\frac12} \]
% 	under the scaling $p_1 \gtrneqsim n^{1/(2\alpha)}(\log(n))^{1/d}$. Equation \eqref{eq:rate:balanced} implies the assertation.
% \end{enumerate}
\end{proof}


\begin{proof}[Proof of Corollary \ref{cor:adaptive:choice:bandwidth}]
The condition $ \bs{p^1} \lesssim  \pmin^d \,\log(\bs{p^1})$ yields that the bandwidth $h_\delta$ is feasible. 
% The considered smoothing parameter $h_\delta$ is feasible because \linebreak $\log(p_1)^{\delta/d}/p_1 \gtrneqsim 1/p_1$ is satisfied. 
Furthermore, Theorem \ref{theorem:estimation:rates} leads to 
\begin{align*}
\sup_{\mu\in\hclass\, Z \in \Pclass} \E_\mu \Big[ \normib{ \muleone - \mu} \Big] = \Oop{ \max\bigg(h_\delta^\alpha, \bigg( \frac{-\log (h_\delta)}{n\bs{p^1}h_\delta^d} \bigg)^{\frac12}, n^{-\frac12}\bigg) }  \,.
\end{align*}
By $\bs{p^1} \gtrsim n^{d/(2\alpha)}\log(n\,\bs{p^1})^{\delta + \zeta}$ we get
\begin{align*}
	h_\delta^\alpha \eqsim \bigg(\frac{\log(\bs{p^1})^{\delta}}{\bs{p^1}}\bigg)^{\alpha/d} \lesssim 
    \bigg( \frac{\log(\bs{p^1})^\delta}{n^{d/(2\alpha)}\log(n\,\bs{p^1})^{\delta + \zeta}}  \bigg)^{\alpha/d} 
    \eqsim \frac{\log(n\,\bs{p^1})^{-\zeta\alpha/d}}{\sqrt n}  
    \lesssim n^{-\frac12}
\end{align*}
and 
\begin{align*}
	\sqrt{\frac{\log(1/h_\delta)}{n\bs{p^1}h_\delta^d}} 
 \eqsim \sqrt{\frac{\log(\bs{p^1})}{n\, \log(\bs{p^1})^\delta} }
 \eqsim \sqrt{\frac{\log(\bs{p^1})^{1-\delta}}{n}} \lesssim n^{-\frac12}\,.
\end{align*}
If we consider $\zeta>0$ we get $h_\delta^\alpha\lessneqsim n^{-1/2}$ in the first display, which yields the negligibility of $\Ionedelta$. If we have in $\delta>1$ the last display shows that also $\Itwodelta$ is negligible compared to $I^{\,n,\bs p , h}_3$. If both inequalities are strict we get the the corollaries second claim.
\end{proof}




==> manageable_processes.tex <==
%
%\begin{definition}[Packing- and Covering Number]\label{def:packingCoveringNumber}
%	Let $(E, \rho)$ be a semimetric space. For a subset $A\subseteq E$ the \textit{packing number} $D(\epsilon, A;\rho)$ for $\epsilon >0 $ is defined by
%	\begin{equation}
%		D(\epsilon, A;\rho) \defeq \max\big\{\# A_0 \mid A_0 \subset A, \rho(s,t) > \epsilon, \; \text{for all different}\; s,t \in A_0 \big\}.
%	\end{equation}
%	The \textit{covering number} $N(\epsilon, A ;\rho)$ for $\epsilon >0 $ is defined by
%	\begin{equation}
%		N(\epsilon, A;\rho) \defeq \max\big\{\# E_0 \mid E_0 \subset E, \inf{s \in E_0},\;\rho(s,t) > \epsilon, \; \text{for all}\; t \in A \big\}.
%	\end{equation}
%\end{definition}
%
%\begin{remark}
%	Those two numbers are related through
%	\begin{equation}
%		N(\epsilon, A; \rho)  \leq D(\epsilon, A ; \rho) \leq N(\epsilon/2, A; \rho) .
%	\end{equation}
%	Compare to \citet[p. 10]{pollard1990empirical}.
%\end{remark}
%
%In the following let $ E = \R^{k_n}$ and $\rho$ be a semimetric on $\R^{k_n}$. 

%\begin{definition}[Envelope]
%
%\end{definition}

%\begin{definition}\label{def:manageability}
%
%\end{definition}


% Proof Philipps Masterarbeit. 




\begin{lemma} \label{lemma:envelope}
	If the weights satisfy \ref{ass:weights:polynom} - \ref{ass:weights:sum}, \ref{ass:weights:lipschitz} and \ref{ass:weights:number:not:vanish} and $p_r \sim p_1$ $\forall\, 1\leq r \leq d$, then the array $(X_{ni})_{n \in \N, 1 \leq i \leq n}$ of processes given by
	\begin{equation*}
		X_{ni}(\bs x)= \frac1{\sqrt n} 	\sum_{\bs j = \bs 1}^{\bs p} \wjp \, Z_i(\bs x_{\bs j})\,, \qquad \bs x \in [0,1]^d \,,
	\end{equation*}
	is manageable with respect to the envelopes $(\Phi_{n})_{n \in \N}= (\Phi_{n1},\ldots,\Phi_{nn})_{n \in \N}$ with 
	\begin{equation*}
		\Phi_{ni}=\frac{C_1}{\sqrt n} \Big( \big|Z_i( \bs 0)\big|+M_1\Big) \,,
	\end{equation*}
	where $M_1$ is given in \ref{ass:Z}. The appropriate capacity bound is 
	\begin{align*}
		\lambda(\epsilon) = \max \bigg(\frac{3^{1/\beta}}{2},C_3C_4,1 \bigg) \epsilon^{-(1+\frac1\beta)} + 2 \,, \qquad \epsilon \in (0,1]\,,
	\end{align*}
	where $\beta$ is given in \ref{ass:Z} as well.
\end{lemma}

The proof can be found in \citet{degras2011simultaneous}.

==> simulations.tex <==
%\subsection{Choice of the bandwidth for $d=1$}

%\subsection{Mean function}

In this section we present the results of a simulation study for dimension $d=1$.  

Since one of the important features of this work is the uniform choice of the bandwidth $h \in (c_0/p,h_0]$ for certain constants $c_0$, $h_0 \in \R_+$ we want to see how those behave and how they have to be chosen in certain examples.
Since also the intervals in which certain rates dominate depend on the unknown parameter $\alpha$ it is of interest how big $p$ needs to be in comparison to $n$ in order to make the bias negligible. \\

%We reconsider the error decomposition from \eqref{eq:decomposition} and the obtained rates of convergence 
%\begin{equation*}
%	\E\bigg[\norm{I_1^{p,h}}_\infty\bigg]=\mc O(h^\alpha),\; \E\bigg[\norm{I_2^{n,p,h}}_\infty\bigg]= \mc O\Bigg(\bigg(\frac{\log(1/h)}{pnh}\bigg)^\frac12\Bigg), \; \E\bigg[\norm{I_3^{n,p,h}}_\infty\bigg]=\mc O_{h\in (c/p,h_0]}\big(n^{-\frac12}\big),
%\end{equation*}
%where the bandwidth $h^\star$ is given by Corollary \ref{cor:optimal:choice:bandwidth}. This exact choice is not required in case that $p$ is large enough in comparison to $n$. \\
%
For the mean function we choose
%
\begin{equation}
	\mu_0(x)= \sin(8\pi(2x-1))\exp(-3\abs{2x-1}), \quad x\in [0,1]. \label{eq:sim:mu}
\end{equation}
We take Gaussian errors and for the individual deviations we use independent Brownian motions. Since we have synchronous design points we directly sample the averaged errors and processes, resulting in  $\bar \e_{j,n} \sim \mc N(0,\sigma^2/n)$ where we take  $\sigma_1^2=0,002^2$ as well as $\sigma_2^2=0,02^2$ and for the individual deviation $\bar Z_{j,n} \sim n^{-1/2} B(t),\, t\in [0,1]$ for a Brownian motion $(B(t))_{t\in[0,1]}$.

\hajo{Noch einen Durchlauf mit geringerer Stichprobengroesse} 
 
We take $n=10000$ and use a local polynomial estimator of order $3$ with the Epanechnikov kernel given by $K_E(x)=3/4(1-x^2)\one_{|x|\leq 1}$. As grid points we choose the equidistant design points $0,1/p,\ldots,(p-1)/p,1$, and repeat the estimation procedure $N=1000$ times. 

Our simulation consist of two steps. First we take a grid of bandwidths $H(p)=\{h_1,\ldots,h_r\}$ for every $p \in \{100,150,200,300,500,750,1000,1500,2000\}$ and estimate the corresponding supremum - errors. For the second part of the simulation we then take the bandwidth with the minimal error for each $p$, and investigate the contributions of each term in the error decomposition \eqref{eq:errordecomp}.  

\begin{figure}
	\centering
	\includegraphics[width=.9\linewidth]{Pictures/opt_h_small_eps.png}
	\caption{Comparison of different bandwidths with $\sigma_1^2$.}
	\label{fig:comp:h:sigma1}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=.9\linewidth]{Pictures/opt_h_medium_eps.png}
	\caption{Comparison of different bandwidths with $\sigma_2^2$.}
	\label{fig:comp:h:sigma2}
\end{figure}

\hajo{Figures bitte neu machen, man kann das in einem schwarz-weiss Ausdruck nicht erkennen}


\hajo{Text neu formulieren}

In figure \ref{fig:comp:h:sigma1} we see that there is no benefit in choosing $h < 0,016$. On the other hand smallest possible values for $h$ where around $3/p$ for each considered $p$. Therefore the interval in which the term $\Ithree$ has the desired rate of convergence and is dominating is approximately $(3/p,0.016]$. Maybe there is a small raise for the smallest possible values in $h$ but those are more visible in figure \ref{fig:comp:h:sigma2}. Here the considered bandwidths were around the same but we can clearly see that a choice of too small bandwidths lead to a bigger error, which can be explained by the dominating of $\Itwo$. However for each $p$ there seems to be an interval of bandwidths where the errors are around the same value, which goes in hand with our theory, since those intervals get larger with the rise of $p$ and all have there upper bound around $0,016$ which is independent of $p$. \\


After we determined appropriate bandwidths in the first part we redo the experiment with those and take a look at the error decompositions and how they evolve in $p$ with fixed $n$ in figure \ref{fig:error:decomp:sigma1:loglog} and figure \ref{fig:error:decomp:sigma2:loglog}. Note that the axis in those are in the logarithm. The picture in both of them can be interpreted in the same way. First the bias is dominating so the increase in $p$ leads to smaller possible bandwidth choices which yields a smaller bias. The bandwidth, and so the bias, stop decreasing at around $p \in [300,500]$. Then the bandwidth seems to be arbitrary and the only effect is the slightly decreasing error term $\Itwo$, which is more notable for $\sigma_2^2$.




\begin{figure}
	\centering
	\includegraphics[width=.9\linewidth]{Pictures/err_decomp_small_eps.png}
	\caption{Error decomposition with $\sigma_1^2$.}
	\label{fig:error:decomp:sigma1:loglog}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=.9\linewidth]{Pictures/err_decomp_medium_eps.png}
	\caption{Error decomposition with $\sigma_2^2$.}
	\label{fig:error:decomp:sigma2:loglog}
\end{figure}

%\subsection{Rates of convergence}


%\subsection{Covariance function}\label{subsec:sim_cov}

\newpage
